SOLD: Slot Object-Centric Latent Dynamics Models for Relational Manipulation Learning from Pixels

Learning a latent dynamics model provides a task-agnostic representation of an agent's understanding of its environment. Leveraging this knowledge for model-based reinforcement learning (RL) holds the potential to improve sample efficiency over model-free methods by learning from imagined rollouts. Furthermore, because the latent space serves as input to behavior models, the informative representations learned by the world model facilitate efficient learning of desired skills. Most existing methods rely on holistic representations of the environment's state. In contrast, humans reason about objects and their interactions, predicting how actions will affect specific parts of their surroundings. Inspired by this, we propose Slot-Attention for Object-centric Latent Dynamics (SOLD), a novel model-based RL algorithm that learns object-centric dynamics models in an unsupervised manner from pixel inputs. We demonstrate that the structured latent space not only improves model interpretability but also provides a valuable input space for behavior models to reason over. Our results show that SOLD outperforms DreamerV3 and TD-MPC2 - state-of-the-art model-based RL algorithms - across a range of benchmark robotic environments that require relational reasoning and manipulation capabilities. Videos are available at https://slot-latent-dynamics.github.io/.

==> figures/environments/figure_all.tex <==
\newcommand\envimgagesize{0.1525\linewidth}

\begin{figure*}[t]
    \centering \sf \scriptsize
    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/ReachSpecific/rollout_00/obs_005.png}}{Reach-Specific}
    \hfill
    \stackunder[2pt]{\stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/ReachSpecificRelative/rollout_00/obs_021.png}}{Reach-Specific-}}{Relative}
    \hfill
    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/PushSpecific/rollout_01/obs_010.png}}{Push-Specific}
    \hfill
    %\stackunder[5pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/PickAndPlaceSpecific/rollout_01/obs_013.png}}{Pick-Specific}
    \stackunder[2pt]{\stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/PickAndPlaceSpecific/rollout_01/obs_013.png}}{PickAndPlace-}}{Specific}
    \hfill
    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/ButtonPress/rollout_00/obs_245.png}}{Button-Press}
    \hfill
    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/CartpoleBalance/rollout_00/obs_014.png}}{Cartpole-Balance}

    \vspace{0.12cm}

    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/ReachDistinct/rollout_00/obs_000.png}}{Reach-Distinct}
    \hfill
    \stackunder[2pt]{\stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/ReachDistinctGroups/rollout_02/obs_019.png}}{Reach-Distinct-}}{Groups}
    \hfill
    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/PushDistinct/rollout_01/obs_009.png}}{Push-Distinct}
    \hfill
    %\stackunder[5pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/PickAndPlaceDistinct/rollout_02/obs_009.png}}{Pick-Distinct}
    \stackunder[2pt]{\stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/PickAndPlaceDistinct/rollout_02/obs_009.png}}{PickAndPlace-}}{Distinct}
    \hfill
    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/Hammer/rollout_00/obs_000.png}}{Hammer}
    \hfill
    \stackunder[2pt]{\includegraphics[width=\envimgagesize,height=\envimgagesize]{figures/environments/FingerSpin/rollout_00/obs_088.png}}{Finger-Spin}
\vspace*{-2mm}
\caption{We evaluate $\MethodAcronym$ on diverse visual environments from (left to right) our multi-object robotic control benchmark, Meta-World~\citep{Yu2019}, and DM-Control~\citep{Tassa2018}.}
	\label{fig:environments}
\end{figure*}

==> figures/non_object_centric_environments/figure.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/non_object_centric_environments/figure.png}
	\caption{\color{blue}
		Training curves for the non-object-centric environments studied in this work.
	}
	\label{fig:non_object_centric_environments}
\end{figure}

==> figures/success_rate_bars/figure.tex <==
\begin{figure}[t]
    \includegraphics*[width=\linewidth]{figures/success_rate_bars/success_rates_chart_new.pdf}
    \caption{Final success rates across the eight evaluated environments.
Overall, $\MethodAcronym$ compares favorably to DreamerV3, showing slight improvements on the \textit{Specific} tasks and a significant performance boost on the \textit{Distinct} variants.}
    \label{fig:final_performance}
\end{figure}

==> sections/05_discussion.tex <==
\section{Discussion}

\paragraph{Pre-training Representations for World Models}
When evaluating for sample-efficiency, we have shifted the required experience of our method to account for the frames used to pre-train the world model.
However, the data used to pre-train the latent representations can come from a static dataset rather than being actively collected during training.
When pre-training structured latent representations leads to improved sample efficiency for the downstream RL tasks, as seen in our experiments, the ability to trade off active interaction data for pre-collected, passive data becomes a valuable option.
Passive data is often more readily available, can be collected in safer conditions, and is generally cheaper to obtain.
Although fine-tuning the encoder-decoder model may be required to account for the state distribution shift introduced by learned behaviors,
this strategy creates an opportunity to pre-train on static dataset to obtain structured latent representations.
In turn, this enables more sample-efficient behavior learning, reducing the amount of actively collected data that is required.





\paragraph{Limitations}
% Stochasticity.
One limitation of our world model is that it generates predictions in a deterministic manner.
This can be a drawback in environments that are inherently stochastic or highly unpredictable.
Incorporating stochasticity into the prediction model is an important avenue for future work.
% SAVi.
A second limitation arises from the object-centric encoder-decoder model we use.
While SAVi performs well on the tasks we evaluated, scaling it to complex real-world data remains a significant challenge.
However, the core ideas of our method are independent of the specific object-centric encoder-decoder model, and future work can easily integrate more advanced models that address these scalability concerns.


\input{figures/savi_finetuning/figure.tex}

==> sections/background.tex <==
\section{Background}
\label{sec:background}

% Should we have a sentence here that puts the background we are going to explain into context so one can more easily understand where SAVi and OCVP fall in the context of our work?


\paragraph{Slot Attention for Video (SAVi):}
%
$\MethodAcronym$ employs SAVi~\citep{Kipf2021}, an encoder-decoder architecture with a structured bottleneck composed of $\NumSlots$ permutation equivariant object embeddings denoted as slots, in order to recursively parse a sequence of video frames $\ImageSeq=\{\ImageT{1}, ..., \ImageT{M}\}$ into their object representations $\SlotSeq=\{\SlotT{1}, ..., \SlotT{M}\}, \SlotT{t} \in \R^{\NumSlots \times \SlotDim}$.
%
%The slots $\SlotT{0}$ are randomly initialized or learned in a data-drive manner.
%
At time $t$, SAVi encodes the input video frame $\ImageT{t}$ into a set of feature maps $\FeatsT{t} \in \R^{\NumFeatLocs \times D_h}$ and uses Slot Attention~\citep{Locatellos2020} to iteratively refine the previous slot representations conditioned on the current features.
%
Namely, Slot Attention performs cross-attention between the slots and image features with the attention coefficients normalized over the slot dimension, thus encouraging the slots to compete to represent feature locations: \\
%
\vspace{-0.1cm}
\begin{align}
	\Attention_t = \softmax_{\NumSlots}(\frac{q(\SlotT{t-1}) \cdot k(\FeatsT{t})^T}{\sqrt{\Dim}}) \in \R^{\NumSlots \times \NumFeatLocs},
	\label{eq:slot_attention}
\end{align}
%
where $q$ and $k$ are learned linear mappings to a common dimension $\Dim$.
%
The slots are then independently updated using a shared Gated Recurrent Unit~\citep{Cho2014GRU} (GRU) followed by a residual MLP:
%
\vspace{-0.1cm}
\begin{align}
	\SlotT{t} = \text{MLP}(\text{GRU}(\Attention_t \cdot v(\FeatsT{t}) , \SlotT{t-1}));
	%
	 \; \; \text{where} \; \Attention_{n,l} = \frac{\Attention_{n,l}}{\sum_{l=0}^{\NumFeatLocs-1}\Attention_{n,l}},
	\label{eq:slot_update}
\end{align}
%
where $v$ is a learned linear projection. The steps described in equations~\ref{eq:slot_attention} and~\ref{eq:slot_update} can be repeated multiple times with shared weights to iteratively refine the slots and obtain an accurate object-centric representation of the scene.
%
Finally, SAVi independently decodes each slot in $\SlotT{t}$ into per-object images and alpha masks, which can be normalized and combined via weighted sum to render video frames.
%
SAVi is trained end-to-end in a self-supervised manner with an image reconstruction loss.







\paragraph{OCVP}
%
We employ the OCVP~\citep{Villar2023} as a forward dynamics model in order to autoregressively predict future object slots conditioned on past object states.
%
%OCVP is a transformer model that decouples the processing of object dynamics and interactions through the use of specialized self-attention variants: \emph{temporal} and \emph{relational attention},
%
%thus leading to interpretable and temporally consistent object predictions while retaining the inherent permutation equivariant properties of the object slots.
OCVP is a transformer model that decouples the processing of object dynamics and interactions, thus leading to interpretable and temporally consistent object predictions while retaining the inherent permutation equivariant properties of the object slots.
%
This is achieved through the use of two specialized self-attention variants:
%
\emph{temporal attention} updates a slot representation by aggregating information from the corresponding slot up to the current time step, without modeling interactions between distinct objects; whereas \emph{relational attention} models object interactions by jointly processing all slots from the same time step.
%
These attention mechanisms can be applied sequentially (OCVP-Seq) or in parallel (OCVP-Par).
%in order to forecast future object slots by modeling the object dynamics and interactions.
%
% TODO: Should I add something about the training procedure?


%
